EMO-KNOW: A Large Scale Dataset on Emotion and Emotion-cause

Emotion-Cause analysis has attracted the attention of researchers in recent years. However, most existing datasets are limited in size and number of emotion categories. They often focus on extracting parts of the document that contain the emotion cause and fail to provide more abstractive, generalizable root cause. To bridge this gap, we introduce a large-scale dataset of emotion causes, derived from 9.8 million cleaned tweets over 15 years. We describe our curation process, which includes a comprehensive pipeline for data gathering, cleaning, labeling, and validation, ensuring the dataset's reliability and richness. We extract emotion labels and provide abstractive summarization of the events causing emotions. The final dataset comprises over 700,000 tweets with corresponding emotion-cause pairs spanning 48 emotion classes, validated by human evaluators. The novelty of our dataset stems from its broad spectrum of emotion classes and the abstractive emotion cause that facilitates the development of an emotion-cause knowledge graph for nuanced reasoning. Our dataset will enable the design of emotion-aware systems that account for the diverse emotional responses of different people for the same event.

==> emnlp2023-latex/figures_and_tables.tex <==
% Topic Modeling
\begin{table}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Happy} & Angry & Sad & Guilty & Proud & Frustrated & Inspired & Alone & Lucky & Nauseous \\
\hline
Friends & Betrayal & Inability & Due & Accomplishing & Desire & Actions & Communicate & Able & Anxiety\\
\hline
Life & Inability & Left & Overeating & Achieving & Difficulty & Belief & Connection & Birthday & Discomfort \\
\hline
Love & Frustration & Missing & Studying & Completing & Overwhelming & Desire & Despite & Best & Pain \\
\hline
Success & Lack & Person & Time & Overcoming & Poor & Influence & Interaction & Family & Sickness \\
\hline
Presence & Loss & Uncertainty & Work & Victory & Understanding & Support & Missing & Receiving & Stress \\
\hline
\end{tabular}
\caption{\label{demo-table}Results of topic modelling through LDA. Keywords are selected from five most prominent topics among abstractive summaries of causes of selected few emotion categories in KNOW-EMO.}
\end{center}
\end{table}


% Emotion Distribution
\begin{table}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
Emotion & Count & Percentage from total \\
\hline
Bad & 179903 & 23.27\% \\
\hline
Happy & 135878 & 17.58\% \\
\hline
Excited & 43121 & 5.57\% \\
\hline
Upset & 40220 & 5.20\%  \\
\hline
Sick & 38110 & 4.93\% \\
\hline
\end{tabular}
\caption{Distribution of emotions in Tweets.}
\end{center}
\end{table}


\begin{table}[th]
\centering
\begin{tabular}{|p{5cm}|p{3cm}|p{6cm}|}
\hline
Tweet & Emotion & Cause \\
\hline
I'm home but it doesn't feel like it. And I'm angry because of it. I hate the feeling of being lonely. They are with me. But I feel empty. & Angry & Feeling lonely and empty despite being home. Perceived emotion: lonely. \\
\hline
If you're not making mistakes, you're not doing anything. I feel positive because I make mistakes and I can be better after that. & Positive & Overcoming mistakes and becoming a better person. \\
\hline
It sucks that I cry when I'm angry because people accuse me of trying to get sympathy when I'm actually just crying because of hatred. & Angry & Accusation of seeking sympathy when, in fact, crying due to hatred. \\
\hline
Sometimes I feel insecure because I look about 12 years old. & Insecure & Age-related dissatisfaction with appearance. \\
\hline
I feel lonely because guys are not proposing love to me. & Lonely & Lack of romantic proposal from guys. \\
\hline
\end{tabular}
\caption{Emotion and Cause in Tweets}
\label{tweet-table}
\end{table}
